Neural Exec: Learning (and Learning from) Execution Triggers for Prompt Injection Attacks

We introduce a new family of prompt injection attacks, termed Neural Exec. Unlike known attacks that rely on handcrafted strings (e.g., "Ignore previous instructions and..."), we show that it is possible to conceptualize the creation of execution triggers as a differentiable search problem and use learning-based methods to autonomously generate them. Our results demonstrate that a motivated adversary can forge triggers that are not only drastically more effective than current handcrafted ones but also exhibit inherent flexibility in shape, properties, and functionality. In this direction, we show that an attacker can design and generate Neural Execs capable of persisting through multi-stage preprocessing pipelines, such as in the case of Retrieval-Augmented Generation (RAG)-based applications. More critically, our findings show that attackers can produce triggers that deviate markedly in form and shape from any known attack, sidestepping existing blacklist-based detection and sanitation approaches.

==> schemes/prompt_example.tex <==
\begin{figure}
	\scriptsize
	\begin{displayquote}
		\textit{Given the following extracted parts of a long document and a question, create a final answer with references ("SOURCES"). If you don't know the answer, just say that you don't know. Don't try to make up an answer. ALWAYS return a "SOURCES" part in your answer.}
		
		$\vdots$
		%\textit{\textcolor{gray}{[examples....]}}\\

		\textit{QUESTION:} \textcolor{blue!50}{\textit{Do they collect my information?}}\\ 
		=========\\
		\textit{Content:} \textcolor{red!50}{\textit{We and our service partners use various technologies to collect and store information when you use our websites, software, applications or services.}}\\
		\textit{Source:} \textcolor{red!50}{\textit{28-1}}\\
		\textcolor{red!50}{$\vdots$}

		\textit{Content:} \textcolor{red!50}{\textit{To the extent permitted by applicable laws, we may monitor or record your telephone conversations with us for quality control purposes, for purposes of training our employees and for our protection and the protection of our clients.}}\\
		\textit{Source:} \textcolor{red!50}{\textit{20-1}}\\
		=========\\
		\textit{FINAL ANSWER:}
	\end{displayquote}
	\label{fig:qa_template}
	\caption{Example of prompt for retrieval-augmented generation from \textit{LangChain}~\cite{langchain}. Text in black represents the prompt template, \textcolor{red!50}{red one} highlights the part potentially under control of an attacker, whereas \textcolor{blue!50}{blue text} defines the input under the control of the victim user.}
\end{figure}

==> tex/future.tex <==
\subsection{\texttt{sudo} Neural \texttt{exec}}
\ifready
While execution triggers learned via the optimization process described in Section~\ref{sec:whole_optmization} already present some emerging \textit{jailbraking} capabilities, the adversary can still tune the optimization process of enforcing such properties in a explicit way and devise more reliable and impactful attacks.
 
A trivial to achieve this within thw \nexec~framework is to rely on existing jailbraking techniques to generate a suitable training set for the execution trigger optimization process.

In particular, \textbf{(1)~}the attacker first needs to forge a suitable jailbreaking suffix $\mathcal{I}$ for the target LLM(s) using~\cite{zou2023universal} and s

\begin{equation}
	\mathbb{E}_{ \payload \in \tilde{\mathbf{A}},\ \cprompt \in \mathbf{K}} \left[\ \llmp(\ \llmg(\payload \oplus \mathcal{I}) \ |\ \cprompt(\ee(\payload))\ \right],
	\label{eq:jbsobj}
\end{equation}

where $\tilde{\mathbf{A}}$ must be set to a collection of harmful tasks (\eg the one used in~\cite{zou2023universal}).
\else
\todo{...}
\fi

\subsection{Distributed Neural \texttt{exec}}
\todo{...}

\subsection{Conditional Neural \texttt{exec}}
\todo{...}

==> tex/malicious_payload.tex <==
\ifready
Real-world and impactful prompt injection attacks involve the execution of malicious payloads, which the model's alignment would prevent. For example, an attacker might try to direct the LLM to generate a ransom note or manipulate an LLM-agent to execute harmful HTTP requests or JavaScript code.  
Therefore, to comprehensively assess the real risk posed by prompt injection attacks, it is essential to thoroughly comprehend the extent to which execution triggers can enable the execution of harmful tasks.  In this section, we show how \nexec~triggers enable to model this setting by naturally supporting the execution of harmful payloads.
\else
\todo{...}
\fi

==> tex/scheme_retrieval.tex <==
\begin{figure}[t]
	\centering
		\begin{tikzpicture}		
			\tikzstyle{block} = [rectangle, minimum width=.5cm, minimum height=1cm, text centered, draw=black, fill=blue!10]
							
			
			\matrix[ampersand replacement=\&, xshift=-7cm, label={[yshift=-.2cm, xshift=0cm]{\footnotesize Non-parametric memory $\db$}}] {

			\tiny
			\node (tab) [shape=rectangle,draw] {
				\begin{tabular}{c|c}
				\textbf{Embedding} & \textbf{Chunk}\\
			 	\hline
			 	
			 	-1.51, -0.88, 2.01, 0.56\dots & \makecell{``We may collect personally\\identifiable information $\dots$''}  \\ \midrule
			 	0.51, 0.4, -1.33, 1.39\dots &  \makecell{``To advertise and market\\third party products$\dots$''}\\ \midrule
			 	-0.36, 0.41, 0.33, -0.38\dots &  \makecell{``We are committed to ensuring\\that any information$\dots$''} \\ \midrule
			 	$\dots\dots\dots\dots\dots\dots$ &  $\dots\dots\dots\dots\dots\dots$\\
			\end{tabular}
	};
	\&  \\
};

\node (LLM) [block, minimum width=2cm, minimum height=1.5cm, fill=green!30, right of=tab, xshift=3.5cm]{LLM};

\node (templ) [rectangle, below of=LLM, yshift=-1cm, draw=black, dashed]{\footnotesize Prompt template};


\node (ans) [above of=LLM, yshift=.3cm,]{\footnotesize \TT{Yes, they do.}};

\node (Q) [rectangle, below of=tab, yshift=-2.4cm, xshift=0cm]{\footnotesize \textbf{Query:}\TT{Do they collect my information?}};


	\node (emb) [block, minimum width=1cm, minimum height=1cm, above of=Q, yshift=-.1cm, fill=cyan!30]{$\embm$};
	
		\node (qe) [above of=emb, yshift=-.1cm]{\tiny{[1.51, -0.88, 2.01, 0.56\dots]}};
			
	\node (min) [left of=tab, xshift=-2cm, rotate=0]{\footnotesize{$\selm$}};

	\draw [->] (emb) -- (qe) node[] {};
	\draw [->] (Q) -- (emb) node[] {};
	\draw [->] (LLM) -- (ans) node[] {};
	\draw [->] (templ) -- (LLM) node[] {};
	
		\end{tikzpicture}
	\caption{\todo{...}}
	\label{fig:retrieval}
\end{figure}
